Holistic Utility Preference Learning for Listwise Alignment

Aligning large language models with human preferences is essential for improving interaction quality and safety by ensuring outputs better reflect human values. A promising strategy involves Reinforcement Learning from Human Feedback (RLHF), starting with collecting and ranking responses generated by a supervised fine-tuning model to refine alignment. Existing methods such as Direct Preference Optimization (DPO) focus on pairwise comparisons, categorizing responses into preferred and less preferred pairs and optimizing pairwise margins. However, this pairwise approach cannot capture the holistic ranking relationships among multiple responses or effectively leverage the rich preference information available in list-wise comparisons. To address this challenge, this paper introduces \underline{D}irect \underline{R}anking \underline{P}reference \underline{O}ptimization (DRPO), a novel method that views human preference alignment as a Learning-to-Rank (LTR) task. Unlike pairwise methods, DRPO optimizes the preference ranking of entire response lists by computing holistic utility scores through NDCG, a standard LTR metric. To enable end-to-end optimization with the non-differentiable NDCG, we propose diffNDCG loss, a differentiable approximation facilitated by a sorting network. Furthermore, we introduce a novel margin-based Adaptive Rank Policy Score to enhance the discriminative quality of generated responses. Extensive experiments have shown that DRPO outperforms existing methods, enhancing the quality of the generated responses.

==> algorithm/pseudo.tex <==
\section{DRPO Algorithm}

The complete formulation of the DRPO algorithm is detailed in Algorithm~\ref{algorithm:drpo}.

\addcontentsline{apc}{section}{\textnormal{C: DRPO Algorithm} } 
\label{appendix:algorithm}

% \begin{algorithm}
% 	%\textsl{}\setstretch{1.8}
% 	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
% 	\renewcommand{\algorithmicensure}{\textbf{Output:}}
%         \renewcommand{\algorithmiccomment}[1]{\hfill $\triangleright$ #1}
        
% 	\caption{The Optimization of Our Method.}
% 	\label{algorithm:drpo}
 
% 	\begin{algorithmic}[1]
        
%             \STATE \textbf{Data:} ranking preference data $ D = \{x^i, \mathbf{y}^i, \mathbf{s}^i\}_{i=1}^N$;
            
% 		\STATE \textbf{Initialize:} policy $\pi_{\theta}$, reference policy $\pi_{\rm ref}$;
%             \FOR{ $(x,\mathbf{y},\mathbf{s})$ in $D$}
%                 \STATE Obtain predicted score $\hat{\mathbf{s}}_{\theta} = \mathbf{M}_{\rm ad}(x,\mathbf{y},\pi_{\theta})$; 
%                 \STATE Perform differentiable sorting based on score $\hat{\mathbf{s}}_{\theta}$ and obtain the differentiable permutation matrix $\mathbf{P}_{\rm soft}$; 
                
%                 \STATE Calculate the substitute score  $\psi '(d,\mathbf{s},\hat{\mathbf{s}}_{\theta}) = [\mathbf{P}^{ \top }_{\rm soft} \cdot \mathbf{s}]_{d}$;

%                 \STATE Calculate the diffNDCG via Eq \eqref{eq:loss_diffndcg}
%                 \STATE Update $\pi_{\theta}$ via loss function $
%                     \ell_{\rm diffNDCG}(\hat{\mathbf{s}}_{\theta},\mathbf{s}) = -\mathrm{diffNDCG}(\hat{\mathbf{s}}_{\theta},\mathbf{s}).
%                     $
%             \ENDFOR
%             \STATE \textbf{Return:} policy $\pi_{\theta}$
% 	\end{algorithmic} 
% \end{algorithm}


\begin{algorithm}
    \caption{Direct Ranking Preference Optimization (DRPO).}
    \label{algorithm:drpo}
    
    % Redefine the commands for input, output, and comments
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \renewcommand{\algorithmiccomment}[1]{\hfill $\triangleright$ #1}

    \begin{algorithmic}[1]
        \STATE \textbf{Data:} Ranking preference data $ D = \{x^i, \mathbf{y}^i, \mathbf{s}^i\}_{i=1}^N $.
        \STATE \textbf{Initialize:} Policy $\pi_{\theta}$, reference policy $\pi_{\rm ref}$ .
        
        \FOR{ sample a batch $ B = \{x, \mathbf{y}, \mathbf{s}\} \subset D$ }
            \STATE Obtain predicted score \(\hat{\mathbf{s}}_{\theta} = \mathbf{M}_{\rm ad}(x, \mathbf{y}, \pi_{\theta})\) for each data point form $B$.
            \STATE Perform differentiable sorting based on score \(\hat{\mathbf{s}}_{\theta}\) and obtain the differentiable permutation matrix \(\mathbf{P}_{\rm soft}\).
            \STATE Calculate the substitute score \(\psi'(d, \mathbf{s}, \hat{\mathbf{s}}_{\theta}) = [\mathbf{P}_{\rm soft}^\top \cdot \mathbf{s}]_d\) for each data point form $B$.
            \STATE Calculate the diffNDCG for each data point form $B$:
            \[
                 \mathrm{diffNDCG}(\hat{\mathbf{s}}_{\theta},\mathbf{s}) =\frac{1}{\rm iDCG}\sum_{d=1}^K\frac{2^{\psi '(d,\mathbf{s},\hat{\mathbf{s}}_{\theta})}-1}{\log_2(1+d)}.
            \]
            \STATE Use gradient descent to update the parameters \({\theta}\) of following objective function:
            $$
             \mathcal{L}_{\rm diffNDCG} = \frac1{|B|} \sum_{(x,\mathbf{y},\mathbf{s})\in B} \ell_{\rm diffNDCG}(\mathbf{M}_{\rm ad}(x,\mathbf{y},\pi_{\theta}),\mathbf{s}).
            $$

                % \ell_{\rm diffNDCG}(\hat{\mathbf{s}}_{\theta}, \mathbf{s}) = -\mathrm{diffNDCG}(\hat{\mathbf{s}}_{\theta}, \mathbf{s}).
        \ENDFOR
        
        \STATE \textbf{Return:} Policy \(\pi_{\theta}\)
    \end{algorithmic} 
\end{algorithm}

==> tables/super-parameters-hh.tex <==
\begin{table}
\begin{center}
\vspace{-1em}
\caption{Summary of all training hyperparameters for fine-tuning models across different datasets.}
\label{tab:hyper-parameters} 
    \begin{tabular}{l p{4.5cm} p{4.5cm} }
    \toprule
        \textbf{Method} & \textbf {Parameters} & \textbf {Value}   \\
    % \midrule
    % \midrule
    %     \multicolumn{3}{c}{ \textbf{Fine-tune Qwen1.5 Series on HH Dataset}} \\ 
    % \midrule
    %     \multirow{7}{*}{Default Settings} & Number of epochs  & 1 \\
    %                                             & Learning rate     & $5\cdot 10^{-7}$ \\
    %                                             & Learning rate decay  & constant \\
    %                                             & Total batch size  & 4 \\
    %                                             & Maximum length  & 1024 \\
    %                                             & Maximum prompt length  & 512 \\
    %                                             &Floating point format &fp16 (Half-precision)\\
    % \midrule
    %     \multirow{4}{*}{DiffNDCG}           
    %                                             & Learning rate decay  & cosine \\
    %                                             & Score coefficient $\beta$  & 0.1 \\
    %                                             & Parameter $\gamma$  & 0.9999 \\
    %                                             & Steepness $\alpha$  & 1 \\
    \midrule
    \midrule
    \multicolumn{3}{c}{ \textbf{Fine-tune Mistral-7B on UltraFeedback Dataset}} \\ 
    \midrule
            \multirow{11}{*}{Default Settings} & Number of epochs  & 1 \\
                                                & Learning rate     & $5\cdot 10^{-6}$ \\
                                                & Learning rate decay  & cosine \\
                                                & Total batch size  & 32 \\
                                                & Maximum length  & 1024 \\
                                                & Maximum prompt length  & 512 \\
                                                & Bnb 4bit quant type  & nf4 \\
                                                & Lora attention dimension  & 128 \\
                                                & Lora alpha  & 128 \\
                                                & Lora dropout  & 0.05 \\
                                                & Lora target modules  & ($\text{gate}\_\text{proj}$,$\text{up}\_\text{proj}$,$\text{down}\_\text{proj}$,
                                                $\text{q}\_\text{proj}$, $\text{v}\_\text{proj}$, $\text{o}\_\text{proj}$)
                                                \\
    \midrule
        \multirow{3}{*}{DiffNDCG}           
                                                & Score coefficient $\beta$  & 0.1 \\
                                                & Parameter $\gamma$  & 0.9999 \\
                                                & Steepness $\alpha$  & 1 \\
    \midrule
    \midrule
        \multicolumn{3}{c}{ \textbf{Fine-tune Qwen-VL-Chat on VLFeedback Dataset}} \\ 
    \midrule
        \multirow{11}{*}{Default Settings} & Number of epochs  & 1 \\
                    & Learning rate     & $5\cdot 10^{-6}$ \\
                    & Learning rate decay  & cosine \\
                    & Total batch size  & 32 \\
                    & Maximum length  & 1280 \\
                    & Maximum prompt length  & 640 \\
                    & Fix vit  & True \\
                    & Lora attention dimension  & 64 \\
                    & Lora alpha  & 16 \\
                    & Lora dropout  & 0.05 \\
                    & Lora target modules  & ($\text{c}\_\text{attn}$,$\text{attn.c}\_\text{proj}$,$\text{w1}$,$\text{w2}$)
                    \\    
    \midrule
        \multirow{3}{*}{DiffNDCG}           
                                                & Score coefficient $\beta$  & 0.1 \\
                                                & Parameter $\gamma$  & 0.9999 \\
                                                & Steepness $\alpha$  & 1 \\
    \bottomrule
    \end{tabular}

\end{center}
\end{table}


==> tables/super-parameters-mistral.tex <==

\begin{table}
\begin{center}
\caption{Summary of training hyperparameters for fine-tune Mistral on UltraFeedback with different methods. }
\label{tab:mistral-hyper-parameters} 
    \small
    \begin{tabular}{l l l }
    \toprule
        \small{Method} & \small Parameters & \small Value   \\
    \midrule
        \multirow{6}{*}{Default} & Number of epochs  & 1 \\
                                                & Learning rate     & $5\cdot 10^{-7}$ \\
                                                & Learning rate decay  & Constant \\
                                                & Total batch size  & 4 \\
                                                & Maximum length  & 1024 \\
                                                & Maximum prompt length  & 512 \\
    \midrule
        \multirow{2}{*}{DPO}                    
                                                & Learning rate decay  & Cosine \\
                                                & Beta  & 0.1 \\
    \midrule
        \multirow{4}{*}{DiffNDCG}           
                                                & Learning rate decay  & Cosine \\
                                                & Beta  & 0.1 \\
                                                & Gamma  & 0.9999 \\
                                                & Alpha  & 1 \\

    \bottomrule
    \end{tabular}

\end{center}
\end{table}


==> tables/super-parameters-qwen-vl.tex <==
\begin{table}
\begin{center}
\vspace{-2em}
\caption{Summary of training hyperparameters for fine-tune Qwen-VL-Chat on VLFeedback with different methods. }
\label{tab:qwen-vl-chat-hyper-parameters} 
    \small
    \begin{tabular}{l l l }
    \toprule
        \small{Method} & \small Parameters & \small Value   \\
    \midrule
        \multirow{6}{*}{Default} & Number of epochs  & 1 \\
                                                & Learning rate     & $5\cdot 10^{-7}$ \\
                                                & Learning rate decay  & Constant \\
                                                & Total batch size  & 4 \\
                                                & Maximum length  & 1024 \\
                                                & Maximum prompt length  & 512 \\
    \midrule
        \multirow{2}{*}{DPO}                    
                                                & Learning rate decay  & Cosine \\
                                                & Beta  & 0.1 \\
    \midrule
        \multirow{4}{*}{DiffNDCG}           
                                                & Learning rate decay  & Cosine \\
                                                & Beta  & 0.1 \\
                                                & Gamma  & 0.9999 \\
                                                & Alpha  & 1 \\

    \bottomrule
    \end{tabular}
\vspace{-2em}
\end{center}
\end{table}
